Efficient Concept Induction for Description Logics

Concept Induction refers to the problem of creating complex Description Logic class descriptions (i.e., TBox axioms) from instance examples (i.e., ABox data). In this paper we look particularly at the case where both a set of positive and a set of negative instances are given, and complex class expressions are sought under which the positive but not the negative examples fall. Concept induction has found applications in ontology engineering, but existing algorithms have fundamental performance issues in some scenarios, mainly because a high number of invokations of an external Description Logic reasoner is usually required. In this paper we present a new algorithm for this problem which drastically reduces the number of reasoner invokations needed. While this comes at the expense of a more limited traversal of the search space, we show that our approach improves execution times by up to several orders of magnitude, while output correctness, measured in the amount of correct coverage of the input instances, remains reasonably high in many cases. Our approach thus should provide a strong alternative to existing systems, in particular in settings where other systems are prohibitively slow.

==> old-concalg.tex <==
\section{Efficient Concept Induction from Instances}\label{sec:concalg}

We now provide a concrete instance of the algorithm described in generic terms in the previous section. We call it the ``Efficient Concept Induction from Instances'' algorithm, ECII (pronounced like ``easy''). We consider again the same three steps, and we assume $\mathcal{O}$ to be an OWL DL ontology \cite{owl2-primer}, i.e., essentially a knowledge base expressed in the description logic $\mathcal{SROIQ}$, although some of our theoretical treatment below will be restricted to OWL EL, i.e.,  $\mathcal{EL}^{\text{++}}$\footnote{For background on description logics, see \cite{BaaderBL05,FOST}}. In the description we will use some parameters, which are natural numbers $n_i$ and $k_i$, and we will refer to them in our exhibition.

In step \ref{item:genalg:1} of the algorithm, we select as additional complex class expressions all class expressions $C$ which are formed by the grammar $C ::= B \mid C_1\sqcap C_2 \mid \exists R.C$ where $B$ is atomic, $R$ is a role, and which contain at most $n_1$ occurrences of the $\sqcap$ symbol and at most $n_2$ occurrences of the $\exists$ symbol (in our system, both $n_1$ and $n_2$ default to $3$, but can be set differently). The rationale behind this choice is simply that we want to remain within the $\mathcal{EL}^{\text{++}}$ language which allows for very efficient (and polynomial time) reasoning. However, if $\mathcal{O}$ is not in OWL EL, then this does not necessarily lead to any advantage, and we could also allow other complex classes from OWL DL which are not in OWL EL -- that does not fundamentally modify the approach.

In step \ref{item:genalg:2} of the algorithm we compute the materialization for all relevant individuals, i.e., the membership of all individuals from the examples in all atomic classes from $\mathcal{O}'$. There are several good algorithms and systems for this, which can be used off-the-shelf. If the ontology $\mathcal{O}$ is already in OWL EL, then this reasoning task is in fact worst-case polynomial in the size of the input. 

In order to explain what we do in step \ref{item:genalg:3} of the algorithm, we need a bit of preparation. First, some definitions.

A \emph{negated disjunct} is a class expression of the form $\neg (D_1\sqcup\dots\sqcup D_k)$, where the $D_i$ are atomic classes from $\mathcal{O}$. A \emph{conjunctive Horn clause} is a class expression of the form $B\sqcap \mathcal{D}$, where $B$ is an atomic class from $\mathcal{O'}$ and $\mathcal{D}$ is a negated disjunct. A \emph{candidate class} is a class expression of the form
$\bigsqcup_{i=1}^m \mathcal{H}_i,$
with conjunctive Horn clauses $\mathcal{H}_i$.

As the term suggests, step \ref{item:genalg:3} of the algorithm will generate solution candidates which involve candidate classes, and will check whether they are solutions. The candidate classes are not the solution candidates; the latter will be defined below.
We restrict ourselves to candidate classes of the mentioned form because 
%two-fold. (1) We use only conjunction, disjunction, and negation because there is an efficient way to check whether individuals fall under these classes, as we will detail below. (2) C
we think that conjunctive Horn clauses can easily be understood by humans, and our intention was to provide solutions in such an easily ingestible form. We will return to this issue in the evaluation section.

We narrow the concept induction problem to the following, which fits our scenarios of interest, as described earlier.

Given an ontology $\mathcal{O}$ (consisting of an ABox and a TBox) over $\mathcal{L}$, an \emph{example} is an individual $a$ together with a set $\mathcal{A}(a)$ of ABox statements (not necessarily contained in $\mathcal{O}$) of the forms $A(a)$, $R(a,b)$ or $B(b)$, for any roles $R$, individuals $b$ and atomic classes $B$. We call two sets $P$ and $N$ of examples the set of \emph{positive} respectively \emph{negative examples} and set $\mathcal{A} = \bigcup_{a\in P\cup N}\mathcal{A}(a)$. We now seek to find a (possibly complex) class expression $\mathcal{S}$ over $\mathcal{L}$ such that $\mathcal{O}\models \mathcal{S}(a)$ for all $a\in P$ (and in this case we say that \emph{$C$ covers $a$}), and also that $\mathcal{O}\not\models \mathcal{S}(b)$ for all $b\in N$. We call $\mathcal{S}$ a \emph{solution} for this learning problem.


Now let $R_1,\dots, R_l$ be all roles occurring in all (positive and negative) examples. A \emph{solution candidate} is a class expression of the form $A \sqcap \bigsqcap_{i=1}^l \exists R_i.\mathcal{C}_i$ or
\begin{align}
A \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\bigsqcup_{j=1}^m (B_{j_i}\sqcap \neg (D_1\sqcup\ldots\sqcup D_{j_{i_k}}))\right)\label{eq:solcand}
\end{align}
where the $\mathcal{C}_i$ are candidate classes and where $A$ and all the $B_j$ and $D_j$ are atomic classes in $\mathcal{O'}$.

In order to now spell out step \ref{item:genalg:3} of the algorithm, we have to present how the solution candidates are generated, and how they are checked whether they are solutions.

Let us first turn to the algorithm for checking whether a solution candidate is a solution. For the following discussion, let us assume for a moment that $\mathcal{O}$ is in OWL EL -- although in general we argue that the same approach can be used for ontologies outside OWL EL.

Now, since the solution candidates contain only roles occurring in the (positive and negative) examples, since we assume for the moment that we are working over OWL EL only, and because of the star shape of the examples, checking whether a solution candidate is a solution can be boiled down to determining the individuals which fall under the candidate classes which are part of a solution candidate: 

Let  
$$\mathcal{C} = \bigsqcup_{j=1}^m (B_j\sqcap \neg (D_1\sqcup\ldots\sqcup D_{j_k}))$$
be such a candidate class. 
We now require some definitions. If $R$ is a role occuring in $\mathcal{A}(a)$ for a (positive or negative) example $a$, then we define \emph{the set of all $R$-fillers of $a$} to be the set $R(a) = \{b\mid R(a,b)\in \mathcal{A}(a)\}$, and if $X$ is a set of individuals then we define \emph{the set of all inverse $R$-fillers of $X$} to be the set $R^-(X) = \{a\mid \text{there is some }b\in X\text{ with }R(a,b)\in \mathcal{A}(a)\}.$ We also set 
%\begin{align*}
$$
\overline{R}^+ = \bigcup_{a\in P} R(a)\qquad
\overline{R}^- = \bigcup_{a\in N} R(a)\qquad
\overline{R} = \overline{R}^+\cup \overline{R}^-
$$
%\end{align*}
for each role $R$.
%
The \emph{extension} $\mathord{\downarrow} B$ of an atomic class $B$ is defined as $\mathord{\downarrow} B = \{b\mid B(b)\in\mathcal{A}\}$.
%$$\mathord{\downarrow} B = \{b\mid \text{there is }B'(b)\in\mathcal{A}\text{ with }B'\sqsubseteq B\}.$$
The extension of the class candidate $\mathcal{C}$ given above is then defined as
$$\mathord{\downarrow}\mathcal{C} = \bigcup_{j=1}^m (\mathord{\downarrow}B_j\cap\setminus(\mathord{\downarrow}D_1\cup\ldots\cup\mathord{\downarrow}D_{j_k})).$$
%
%We now have the following -- see the supplementary material for the proof.
%
%\begin{proposition}\label{prop:correctness}
%Let $\mathcal{O}$ be in OWL EL. Let $\mathcal{C}$ be a candidate class and let $b$ be any $R$-filler, for any $R$, for any example individual. 
%Then $\mathcal{O'}\cup \mathcal{A}\models \mathcal{C}(b)$ if and only if $b\in\mathord{\downarrow}\mathcal{C}$.
%\end{proposition}
%
%\begin{proof}
%The direction from right to left is obvious. For the opposite direction, recall the well-known fact that, for any $\mathcal{EL}^{++}$ knowledge base $\mathcal{K}$, atomic classes $A_1$, $A_2$ and individual $a$, we have that $\mathcal{K}\models (A_1\sqcup A_2)(a)$ holds if and only if at least one of $\mathcal{K}\models A_1(a)$ or $\mathcal{K} \models A_2(a)$ holds -- this is a direct consequence of the inability to express disjunctive inferences in $\mathcal{EL}^{++}$.
%\end{proof}
Now if 
$$\mathcal{S} = A \sqcap \bigsqcap_{i=1}^l \exists R_i.\mathcal{C}_i$$
is a solution candidate, then let
$$\mathord{\downarrow}\mathcal{S} = \mathord{\downarrow}A \cap \bigcap_{i=1}^l R_i^-(\mathord{\downarrow}\mathcal{C}_i).$$

%We now have the following -- see the supplementary material for the proof.
%The following follows now easily.
%\input{theorem1}

%\bigskip

Let us now turn to the generation of solution candidates. Essentially, the set of all possible solution candiates can be understood as a search space, within which we want to locate solutions or at least approximate solutions which are highly accurate in terms of coverage or not of the examples.  
%which we traverse, at each step checking how good the current solution candidate is, and deciding where to go next in the search space. Our method -- as 

The DL-Learner system, which is our primary comparison, is based on traversing the search space by means of a so-called \emph{refinement operator}, an idea borrowed from Inductive Logic Programming \cite{NienhuysW97}: Given a solution candidate, the refinement operator produces a set of new solution candidates. These are all assessed as to their accuracy in terms of coverage or not of the examples, and the best are kept and the process is iterated. The DL-Learner system calls an external reasoner each time the accuracy of a candidate solution is to be assessed.

Our approach, however, dispenses of the need to call an external reasoner as discussed above.
% given the result in Theorem \ref{theo:solutioncheck}.
We could now of course use a refinement-operator approach to iteratively create solution candidates and check them. 
% in accordance with Theorem \ref{theo:solutioncheck}.
However since accuracy assessment in our setting is very quick, and since our solutions are of very specific forms, we instead opted for a direct assembly of solution candidates from its parts, as described in the following.

Recall that our solution candidates are of the form (\ref{eq:solcand}).
%\begin{align*}
%\mathcal{S} &= A \sqcap \bigsqcap_{i=1}^l \exists R_i.\mathcal{C}_{i}\\
%&= A \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\bigsqcup_{j=1}^m (B_{j_i}\sqcap \neg (D_1\sqcup\ldots\sqcup D_{j_{i_k}}))\right),
%\end{align*}
%where the $\mathcal{C}_i$ are candidate classes and where $A$ and all the $B_j$ and $D_j$ are atomic classes in $\mathcal{O'}$.
%and note that a solution candidate consists of a single atomic class for $l=0$, and that similarly $j_{i_k}=0$ means that the corresponding conjunctive Horn clause consists only of a single atomic class. 
Our algorithm for constructing solution candidates consists of three consecutive steps: (I) Select a set of conjunctive Horn clauses. (II) Select a set of candidate classes constructed from the selection in step (I). (III) Select a set of candidate solutions constructed from the selection in step (II). 

These three steps, each of which we are going to describe in detail shortly, depend on five user-defined parameters $k_1,\dots,k_5$ which are natural numbers. Their default values are $k_1=k_2=k_3 = 3$ and $k_4=k_5=50$, but they can be changed by the user. 

(I) For every role $R$ occuring in the examples, set 
$
N_R= \{B\mid B \text{ is an atomic }\text{class in }\mathcal{O}'\text{ and there is }b\in\overline{R}\text{ with }b\in \mathord{\downarrow}B\}.
$
Then, for each role $R$, construct the set $H_{0,R}$ of all conjunctive Horn clauses, each of which contains only atomic classes from $N_R$, and at most $k_1$ of such classes each.

Then, for each $H\in H_{0,R}$, calculate the accuracy of $H$ as
$$\alpha_1(H) = \frac{|\overline{R}^+\cap \mathord{\downarrow}H| + |\overline{R}^-\setminus \mathord{\downarrow}H|}{|\overline{R}|}.$$

Finally, let $H_R$ be the set of the $k_4$ conjunctive Horn clauses from $H_{0,R}$ which have the highest accuracy; if two clauses are of the same accuracy, then we use those of shorter length, where length is measured in the number of atomic classes occuring in the conjunctive Horn clause. $H_R$ is the set of conjunctive Horn clauses selected in this step.

(II) For every role $R$ occuring in the examples, set $C_{0,R}$ to be the set of candidate classes assembled as disjunctions of maximally $k_2$ conjunctive Horn clauses from $H_R$ each. 

Then, as before, we select the set $C_R$ of the $k_6$ candidate classes from $C_{0,R}$ which have the highest accuracy, and if two candidate classes are of the same accuracy, then we use those of shorter length. 
 
(III) Construct the set of candidate solutions 
$S_0 = \left\{A \sqcap \bigsqcap_{i=1}^{k_3} \exists R_i.\mathcal{C}_{i}\middle| \mathcal{C}_{i}\in C_{R_i}, A\text{ an atomic class} \text{ in } \mathcal{O}'\right\}.$
Our output set $S$ consists of the best candidate solutions from $S_0$ again selected by means of highest accuracy and shortest length, where the accuracy for each $C\in S$ is %computed as 
$$\alpha_2(C) = \frac{|P\cap \mathord{\downarrow}C| + |N\setminus \mathord{\downarrow}C|}{|P\cup N|}.$$

Let us make some remarks. In (I), we essentially brute-force the search for good conjunctive Horn clauses for each set of $R$-fillers, and $N_R$ are all the classes relevant for these $R$-fillers. Accuracy is simply measured by coverage of $R$-fillers from the positive examples and non-coverage of the $R$-fillers from the negative examples, as a quotient with the number of all $R$-fillers. Length as a tie-breaker makes sense because we retain our intention to produce human-interpretable solutions, i.e., simple solutions are preferred. The size of $H_{0,R}$ is of course exponential in $k_1$, but this simply reflects the nature of the search space. Likewise, step (II) is exponential in $k_2$, and step (III) is exponential in $k_3$. The accuracy measure in step (III) is essentially the same as the one in steps (I) and (II), just that now we are looking at the examples, instead of the $R$-fillers. The required computations in all steps are straightforward arithmetic or set operations. 
% in the light %of Proposition \ref{prop:correctness} and of Theorem \ref{theo:solutioncheck}.

Due to the already mentioned deliberate decision to trade completeness for runtime improvements, our approach will of course not necessarily find all solutions or best solutions. It is to be understood as a heuristics which delivers a favorable trade-off between accuracy and speed, as we argue in the evaluation section below.


%only old dumps below this


%We chose to focus on OWL EL because it is of relatively low worst-case complexity -- polynomial in the size of the ontology -- and thus lends itself to efficient reasoning. Furthermore, it has some theoretical properties which make it particularly suitable for our setting, as can be seen from some of the detailed arguments which we are making below. We will discuss later how to deal with ontologies outside OWL EL in an approximate manner, and there will be corresponding evaluations in Section \ref{sec:eval}.

%In this vein, since we are already approximating the underlying reasoning procedure, it makes sense to further explore this aspect. E.g., if the given ontology is not in OWL EL, then we could e.g. choose to ignore the axioms outside OWL EL, and perform reasoning over the remaining axioms only. While any additional such approximate reasoning procedure \cite{RudolphTH08} potentially decreases accuracy, this can again be weighed against the runtime improvements, as required by the application scenario.



%Then the refinement operator $\varrho$ is defined as specified in Figure \ref{fig:ref-op}.
%\begin{figure}[t]
%\begin{align*}
%\varrho(\mathcal{S}) = &\left\{A' \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\bigsqcup_{j=1}^m \mathcal{C}_{j_i}\right)\middle| A'\prec A\right\} \\ 
%&\cup\Biggl\{ 
%\mathcal{S} \sqcap \exists R_{l+1}.\top \Bigg| R_{l+1}\text{ occurs in }P\cup N\text{ but not in }\mathcal{S}\Biggr\}\\ 
%&\cup\Biggl\{A \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\left(\bigsqcup_{j=1}^m \mathcal{C}_{j_i}\right)\sqcup B'\right)\Bigg| B'\not= B_{j_i}\text{ for all }j_i\text{ and }B'\text{ is}\\ &\qquad\text{a sibling of some }B_{j_i}   
%\Biggr\}\\  
%&\cup\Biggl\{A \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\bigsqcup_{j=1}^m (B'\sqcap \neg (D_1\sqcup\ldots\sqcup D_{j_{i_k}}))\right) \Bigg| B'\text{ replaces one }B_{j_i}\\ &\qquad\text{where }B'\prec B_{j_i} \Biggr\}\\
%&\cup\Biggl\{A \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\bigsqcup_{j=1}^m ( B_{j_i}\sqcap \neg (D_1\sqcup\ldots\sqcup D'\sqcup\ldots\sqcup D_{j_{i_k}}))\right) \Bigg|  D'\text{ replaces}\\ &\qquad\text{one }D_x\text{ with }D_x\prec D'\Biggr\}\\
%&\cup\Biggl\{A \sqcap \bigsqcap_{i=1}^l \exists R_i.\left(\bigsqcup_{j=1}^m ( B_{j_i}\sqcap \neg (D_1\sqcup\ldots\sqcup D_{j_{i_k}}\sqcup D'))\right) \Bigg|\text{there is some}\\ &\qquad R_i\text{-filler }b\text{ with }D'(b)\in N\text{ and }D'\not\sqsubseteq D_x\text{ for any }x\in\{1,\dots,j_{i_k}\}\Biggr\} 
%\end{align*}
%\caption{Refinement operator definition}\label{fig:ref-op}
%\end{figure}

%The refinement operator is used to traverse the search space of all solution candidates, starting with $\top$, effectively creating a search tree. Which nodes to expand next is guided by a heuristics. While creating the search tree, the newly created solution candidates are checked whether they constitute solutions, and if not, how good they are as relative solutions.



==> theorem1.tex <==
\begin{theorem}\label{theo:solutioncheck}
    Let $\mathcal{O}$ be in OWL EL. A solution candidate $\mathcal{S}$ is a solution if and only if both of the following hold.
    \begin{compactenum}
        \item $a\in \mathord{\downarrow}\mathcal{S}$ for all positive examples $a$ in $P$.
        \item $a\not\in \mathord{\downarrow}\mathcal{S}$ for all negative examples $a$ in $N$.
    \end{compactenum}
\end{theorem}

According to Theorem \ref{theo:solutioncheck}, checking whether a solution candidate is a solution can be done simply by means of a number of straightforward set-theoretic operations, which is easily implemented.

Of course, Theorem \ref{theo:solutioncheck} has been established with $\mathcal{O}$ being in OWL EL. If $\mathcal{O}$ is not in OWL EL, then in general Theorem \ref{theo:solutioncheck} does obviously not hold. However, we can consider the checking of a solution candidate, by checking whether conditions 1. and 2. from the theorem hold,
%\begin{enumerate}
%\item $a\in \mathord{\downarrow}\mathcal{S}$ holds for all positive examples $a$ in $P$ and
%\item $a\not\in \mathord{\downarrow}\mathcal{S}$ holds for all negative examples $a$ in $N$
%\end{enumerate}
to be an approximate reasoning procedure \cite{RudolphTH08} for the full entailment problem. As a result, we do of course sometimes get incorrect assessments, and whether or not this is a reasonable thing to do depends on the use case, and in particular on the question whether the runtime improvments for the use case outweigh the severity of the reasoning mistakes we get in return. We will better understand this trade-off when we discuss our evaluation results.
